Summarized Causal Explanations For Aggregate Views (Full version)

SQL queries with group-by and average are frequently used and plotted as bar charts in several data analysis applications. Understanding the reasons behind the results in such an aggregate view may be a highly non-trivial and time-consuming task, especially for large datasets with multiple attributes. Hence, generating automated explanations for aggregate views can allow users to gain better insights into the results while saving time in data analysis. When providing explanations for such views, it is paramount to ensure that they are succinct yet comprehensive, reveal different types of insights that hold for different aggregate answers in the view, and, most importantly, they reflect reality and arm users to make informed data-driven decisions, i.e., the explanations do not only consider correlations but are causal. In this paper, we present CauSumX, a framework for generating summarized causal explanations for the entire aggregate view. Using background knowledge captured in a causal DAG, CauSumX finds the most effective causal treatments for different groups in the view. We formally define the framework and the optimization problem, study its complexity, and devise an efficient algorithm using the Apriori algorithm, LP rounding, and several optimizations. We experimentally show that our system generates useful summarized causal explanations compared to prior work and scales well for large high-dimensional data

==> extensions.tex <==
\section{Extensions}\label{sec:extensions}

\paratitle{Support for multi-relation databases}
For a multi-relation database, this definition needs to be augmented since the units on which the treatment is being applied have to be pre-defined, and in our scenario, the treated units may vary depending on the chosen treatment. For example, consider an academic database with authors, papers, and institutes, where each author can have multiple papers and each paper can have multiple authors. Also consider the query grouping institutes by their average prestige (prestige is an attribute in the author table). We could examine treatments that affect the authors like changing their field, or treatments that affect papers like changing the venue in which they were published. Therefore, we have to retrace the units for each such examined treatment and examine its CATE. 

\begin{itemize}
    \item how to operate without a causal DAG - estimate the correlations?
    \item How to operate on a multi-relation dataset? such as DBLP
    \item  what to do if the SUTVA assumption does not hold? (e.g., flights)
    \item other aggregates (sum, count)
 
\end{itemize}

\vspace{2mm}
% \brit{Possible Extensions}:
\begin{itemize}
    \item Removing the assumption we have the causal DAG 
    \item Explanations can use ranges or any other operator (not only equality) - the search space becomes much bigger
    \item explanations may not be uniform - tuples with different values for the outcome. In this case we want to maximize uniformity as well. 
    \item Removing the requirement to explain the entire view
\end{itemize}


==> response.tex <==
\twocolumn

\section*{Response to the Reviewers}
\noindent \textbf{Dear reviewers,}

\noindent 
We would like to express our gratitude to the reviewers for their valuable feedback, which helped us improve our paper.
In response to the reviewers' comments, we focused on addressing four main areas of improvement:
(1) improvement of the experimental evaluation by including additional baselines and quantitative measures of accuracy, (2) adding stronger justifications for the used assumptions, (3) adding clarifications about the pattern mining and the sampling algorithms, and (4) adding explanations of the rationale behind some design choices. 
To address these issues, we have provided a detailed explanation of our responses to the main concerns that were raised by all reviewers. We have also addressed each reviewer's comments individually.

Updates made in response to specific comments are highlighted in the revised manuscript using the following colors:
\begin{itemize}
\item \common{Changes mentioned by multiple reviewers in Plum}
\item \reva{Reviewer 1 in Blue}
\item \revb{Reviewer 2 in Magenta}
\item \revc{Reviewer 3 in Purple} 
\end{itemize}


\subsection*{Main Changes by the Meta Review}
\textbf{Required changes:} {\em The required changes refer to various issues in the paper. In short, they include (a) improvements and enhancements of the experimental evaluation (such as comparison with more appropriate baselines, especially causal ones, quantitative measures of quality and accuracy), (b) stronger justification of some of the assumptions regarding the scope of the proposed framework, (c) clarifications about the pattern mining and the sampling algorithms and (d) clearer explanations of the rationale behind some design choices. All revisions required for acceptance are described clearly in Q14 in the reviews.}


\vspace{1mm}
\noindent
% {\bf{(\colorbox{pink}{Point \textrm{1}}) Additional Experiments}}. 
{\bf{(\colorbox{pink}{Point \textrm{1}}) Improvements and enhancements of the experimental evaluation}}. 
\common{
Following the reviewers' suggestions, we have expanded our experimental study, including adding two baselines. We summarize the main changes here:


$\bullet$ \textbf{Adding a causal baseline.}
We added to our experiments an additional causal baseline algorithm {\bf (please see \cref{subsec:setup})}. 
In particular, we added {\bf \xinsight}~\cite{abs-2207-12718}, a framework that identifies both causal and non-causal patterns to explain the differences between two groups of tuples in the result of a group-by query. To compare against our solution, we generate an explanation for the entire aggregate view by comparing all $\binom{|Q(D)|}{2}$ pairs of groups. \xinsight\ also discovers a causal DAG and uses it to identify the causal explanations. For a fair comparison, we skipped the causal discovery phase and employed the same causal DAG used by \algoName. We next summarize our main findings. 



(1) As mentioned above, to generate an explanation for the entire view, we utilized \xinsight\ to explain the differences between \emph{all pairs of groups}. As a result, this approach yields comprehensive explanations. For instance, in the \so\ (StackOverflow data) scenario, the explanation encompassed all country pairs comparisons (20 choose 2), resulting in an explanation of size exceeding 500KB (provided in \cite{fullversion}). In the \accidents\ scenario, because of the vast number of cities (over
50,000) it was infeasible for \xinsight\ to generate an explanation within our time cutoff (3 hours). 

(2) Similar to \algoName, \xinsight\ focuses on patterns involving attributes that causally influence the outcome, such as \textsf{Education} and \textsf{Gender} in \so. However, we argue that these explanations offer distinct perspectives on the
query results. 
Whereas \algoName\ finds joint treatments for sets of groups, \xinsight\ returns patterns that explain the difference between two groups. 
For instance, in \so, \xinsight’s explanation sheds light on the
substantial variance in average salaries between the US and Poland,
highlighting differences in the distribution of role types. In the US,
there is a prevalence of ML specialists and C-level
executives, while Poland has a higher concentration of Back-end
developers and DevOps specialists. Conversely, \algoName\ explanation uncovers \emph{commonalities} among various country groups, such as the positive impact of being under the age of 35 on salaries across all
European countries. Therefore, these two solutions can be viewed
as complementary efforts, each revealing different causal insights behind aggregate views.


% Nevertheless, \algoName\
% can be customized to exclusively elucidate the distinctions between
% two groups in the query result, by focusing on a particular segment of the aggregated
% view through the use of a WHERE clause in the query (selecting
% only the tuples associated with these two groups). In contrast,
% \xinsight\ lacks a straightforward extension for explaining the entire
% aggregated view via a summarized, concise explanation.
(3) Nevertheless, if the query returns only two groups, \algoName\ 
can find treatments (patterns) that explain the difference between their outcomes. 
In the example about the US and Poland, the returned treatment by \algoName\ was similar to the one obtained from \xinsight (e.g., \algoName\ also recognized that having a C-level executive position is the treatment with the highest positive effect on respondents from the US). 
In contrast, in the presence of multiple groups in the query result, 
\xinsight\ lacks a straightforward extension for generating a summarized explanation for the entire aggregate view.

$\bullet$ \textbf{Adding another variant of the Explanation Table baseline:}
We have included another variant of the {\bf \exptable\ algorithm} \cite{Gebaly+2014-expltable}, referred to as \exptableG, to consider a group-by SQL query ({\bf full details are given in \cref{sec:experiments}}). This variant considers the grouping patterns found by \algoName\ and reports the pattern found by \exptable\ separately for each grouping pattern. 
Our findings suggest that, although this variant addresses the limitation of \exptable\ in capturing variations among groups in the query result, it falls short in providing causal explanations. For example, in the \so\ scenario, as \exptable, \exptableG\ identified \textsf{YearsCoding} as a significant factor for multiple grouping patterns, indicating that individuals with over 30 years or less than 2 years of coding experience tend to have lower salaries. This aligns with our observation related to being a student or being over 55, which also leads to reduced salaries. However, \textsf{Age} and \textsf{Role} have a more substantial causal effect on salary than \textsf{YearsCoding}. This underscores the fundamental difference between \exptable, which prioritizes patterns with high information gain, and our approach, which focuses on identifying patterns with strong causal effects.





$\bullet$ \textbf{Adding experiments over synthetic data:}
To evaluate the accuracy of the \algoName\ algorithm, we included experiments conducted over syntactic data where the ground truth is known. 
% In this setting, there are multiple grouping and treatment patterns to be considered. Due to our pruning optimizations, we anticipate that both the treatment and grouping pattern mining algorithms will exclude certain patterns from consideration. 
{\bf To assess the effectiveness of the grouping and treatment patterns mining algorithms compared to the exhaustive \bruteforce\ baseline, we report their precision and recall.}
We summarize our main findings below ({\bf please see Section \ref{subsec:quality_eval}} for full details).


\textbf{Grouping patterns}: We manipulate the count of attributes utilized for grouping patterns, thereby controlling the number of potential grouping patterns. To assess the precision and recall of the grouping pattern mining algorithm (\cref{subsec:grouping_patterns}), we compare the tuples covered by the grouping patterns chosen by \algoName\ against those covered by the \bruteforce\ algorithm. The results are shown in {\bf new Figure {\bf \ref{fig:precision_recall}(a)}}. Our results show that when the count of potential grouping patterns is relatively low (up to 20 patterns), our grouping patterns mining algorithm selects patterns that cover the same tuples as \bruteforce. As the number of grouping patterns to consider increases, the algorithm prunes certain patterns, leading to a decrease in precision and recall. Nevertheless, these scores consistently remain high (above 0.78), signifying that \algoName\ and \bruteforce\ cover nearly the same tuples. 

\textbf{Treatment patterns}: To assess the performance of the treatment pattern mining algorithm (\cref{subsec:treatment_patterns}), we consider a fixed count of 20 grouping patterns, where both \algoName\ and \bruteforce\ selected the same grouping patterns. We then evaluated the precision and recall of the treatment mining algorithm in comparison to the treatments chosen by \bruteforce. Specifically, we compared the tuples identified as the treated group by \algoName\ with those defined as the treated group according to \bruteforce. We report average precision and recall across all grouping-treatment pattern combinations. The results are shown in {\bf new Figure \ref{fig:precision_recall}(b)}. Observe that the recall remains consistently high, irrespective of the number of treatment patterns. This suggests that the treated group according to \bruteforce\ is always encompassed by the treated group identified by \algoName. In contrast, precision decreases as the count of treatment patterns increases. This signifies that the treated group, according to \algoName\ may contain some irrelevant tuples. This is due to the pruning optimizations employed by \algoName, which prevent it from materializing "long" patterns. However, even with many treatment patterns, the precision consistently exceeds 0.78.
}

\vspace{1mm}
\noindent
% {\bf{(\colorbox{pink}{Point \textrm{2}}) Assumptions Justification}}.
{\bf{(\colorbox{pink}{Point \textrm{2}}) Stronger justification of some of the assumptions regarding the scope of the proposed framework}}.
\common{
We extended our discussion regarding the limitations of \algoName\ and elaborated on the assumptions we have made.

$\bullet$ \textbf{Adding a discussion on limitations:}
We have revised {\bf \cref{sec:conc}} and emphasize that our framework currently supports a single-relation database with no dependencies among the tuples. The rationale behind this assumption is to ensure the SUTVA assumption~\cite{rubin2005causal} (as mentioned in \cref{sec:prelim}) holds.
SUTVA is a crucial assumption in causal inference, asserting that the treatment of one unit should not impact the outcome of another.
Even for a single-table database with dependencies among tuples, this assumption no longer holds. For example, in the popular {\em Flights} dataset \cite{kaggle_flights} for flight delay, the delay of one flight has an impact on subsequent flights using the same aircraft, and is also dependent on flights leaving and arriving in the same airport. Consequently, attempting to compute the causal effect of a treatment on such datasets would result in invalid inference. 


When dealing with a single table, treatment patterns are well-defined, and grouping patterns are defined with attributes with functional dependencies to the grouping attributes. However, extending these concepts to multi-table scenarios, where grouping attributes, treatments, and outcomes may originate from different tables, poses several challenges due to the need to address many-to-many relationships and patterns spanning multiple tables. Additionally, in multi-table databases, intricate dependencies among tuples can exist, potentially violating the SUTVA assumption.
While previous work \cite{SalimiPKGRS20,galhotra2022hyper} extended causal models to accommodate multi-table data and employed them for hypothetical query answering, they have not studied the problem of explaining aggregate views. Extending our framework to support multi-table databases with complex dependencies is an important future work and we include it in \cref{sec:conc}. Note that prior work on causal explanations \cite{abs-2207-12718, youngmann2022explaining, salimi2018bias} has primarily focused on single tables as well.








$\bullet$ \textbf{Dependence on causal DAGs:}
As we demonstrate in the revised \cref{subsec:exp-sensitivity}, our results depend on the input causal DAG. To further investigate this aspect, we expanded our experiments to examine the performance with scenarios involving the use of naive causal DAGs. In particular, we compared the results with a causal DAG wherein all attributes are directly linked to the outcome variable via edges, and no other edges exist within the DAG, similar to the approach taken by previous work~\cite{GalhotraGRS22}.
Our findings reveal that even the employment of basic causal discovery algorithms (we experimented with the PC~\cite{spirtes2000causation}, FCI~\cite{spirtes2000causation}, and LiNGAM~\cite{shimizu2006linear} algorithm) produces superior results when compared to the absence of any assumed causal DAG. It is worth noting that causal DAGs can originate from various sources, including domain knowledge, GPT, or existing causal discovery methods. This experiment illustrates that while our results do rely on the input causal DAG, the currently available methods for deriving such a DAG are capable of producing meaningful results (full details are given in {\bf \cref{subsec:exp-sensitivity}}).



$\bullet$ \textbf{Supporting AVG:} 
We have moved the justification for our approach of supporting only the AVG aggregation function to {\bf Section \ref{sec:conc}}. 
In particular, restricting to AVG is fundamental for causal explanations unlike non-causal methods.
Our framework aims to find summarized \underline{\em causal explanations} for the query answers in $Q(D)$ using the concept of CATE discussed in Section~\ref{sec:prelim}. The causal estimates by CATE as shown in Eq.~(\ref{eq:cate}) and (\ref{eq:conf-cate}), inherently use {\em expectations, i.e., weighted average}. Thus, CATEs can be used when considering the aggregate average on the outcome column $Y$. Aggregate functions like {\tt SUM} or {\tt COUNT} depend on the {\em number of units} satisfying the conditions in Eq.~(\ref{eq:cate}) and (\ref{eq:conf-cate}), which does not have a correspondence with the estimate of causal effect (except that larger groups might reduce variance in the estimate). While other non-causal work on explanations or summarizations for query answers \cite{wu2013scorpion, roy2014formal, miao2019going, li2021putting, lakshmanan2002quotient, wen2018interactive} can support other aggregate functions, existing methods based on causal estimates focus on average as well \cite{salimi2018bias,youngmann2022explaining,abs-2207-12718}.
}




\vspace{1mm}
\noindent
% {\bf{(\colorbox{pink}{Point \textrm{3}}) Clarifications about the Algorithms}}.
{\bf{(\colorbox{pink}{Point \textrm{3}}) Clarifications about the pattern mining and the sampling algorithms}}.\common{
We {\bf revised \cref{sec:algo}} to better explain our proposed algorithms and now emphasize that a brute-force approach considers all grouping and treatment patterns and results in long runtimes (as we demonstrate in our experimental study). Instead, the \algoName\ algorithm adapts the Apriori algorithm~\cite{agrawal1994fast} to mine frequent grouping patterns (the coverage of such patterns is monotone) as a heuristic for finding promising grouping patterns that are short (we ignore the rest). To mine treatment patterns (which are non-monotone for CATE), we adopt a lattice traversal approach and use a greedy heuristic materializing only promising treatment patterns. Both steps can result in a non-optimal solution. In \cref{sec:experiments} we compare \algoName\ against Brute-Force and show that while \algoName\ is much faster, the difference in results (in terms of explainability, coverage, and accuracy) is modest.


As for the sampling optimization, we have {\bf revised the text in \cref{subsec:treatment_patterns}} as follows:
To decrease running times, we use a fixed-size random sample of tuples to estimate CATE values (lines 3, 8) and investigate the impact of sample size on runtime and accuracy. Random sampling of tuples is done only for evaluating CATE values and not for mining patterns. Our experimental study shows that using a random sample size of $1$ million tuples yields CATE estimates that closely match those obtained from the entire dataset. (Full details are given in the {\bf revised Section \ref{subsec:exp-sensitivity}}).
}


\vspace{1mm}
\noindent
% {\bf{(\colorbox{pink}{Point \textrm{4}}) Discussions on design choices}}.
{\bf{(\colorbox{pink}{Point \textrm{4}}) Clearer explanations of the rationale behind some design choices}}.
% Following the reviewers' suggestions, we provide clearer explanations of the rationale behind some design choices.
\common{
Following the reviewers' suggestions, we have made the following revisions.


$\bullet$ \textbf{Positive and negative treatments:}
{\bf \cref{subsec:problem}} now includes a discussion about the usefulness of both treatment types in our setting.  
Given an outcome variable (e.g., income), positive explanations correspond to treatments that have an impact on making its value higher (what increases income), and negative explanations are treatments that make its value lower (what reduces income). These positive/negative treatments can vary for different groups (as illustrated in Figure~\ref{fig:so-explanation}). Thus, both may be valuable. Consequently, our proposed framework supports both. In a future prototype with a user interface, analysts have the flexibility to choose whether they want to view one or both types of explanations and even top-k positive/negative treatments for a grouping pattern.
This helps understand the cause of both high and low values of outcomes for different groups without explicitly asking for explanations for high and low values as done in previous work \cite{wu2013scorpion, roy2014formal, miao2019going, li2021putting}.


% \texttt{To generate positive and negative patterns for each grouping pattern, we slightly vary the optimization objective in Definition~\ref{def:problem}. 
% For a %subgroup of query answers defined by a 
% grouping pattern $\pattern_g$, we find a treatment pattern $\pattern^+_{g, tp}$ with the {\em highest explainability value of $(\pattern_g, \pattern^+_{g, t})$} ($\pattern^+_{g, t}$ is called a {\em positive treatment pattern} for $\pattern_g$). A {\em negative treatment pattern} $\pattern^-_{g, t}$ is defined similarly using the lowest explainability value. 
% In our system, for each grouping pattern $\pattern_g$ we compute the sum of absolute values of two explainabilities: 
% $|Explainability(\pattern_g, \pattern^+_{g, t})| + |Explainability(\pattern_g, \pattern^-_{g, t})|$.
% We treat this sum as the weight of the explanation pattern combination $(\pattern_g, \pattern^+_{g, t}, \pattern^-_{g, t})$ and return top-$k$ explanations that satisfy the constraints in Definition~\ref{def:problem}. }



$\bullet$ \textbf{Continuous variables:}
We include the following discussion in {\bf \cref{sec:conc}}: 
We note that attributes used for defining the grouping patterns must be categorical, as they need to exhibit a functional dependency with the grouping attribute. However, attributes used to define treatment patterns can take either continuous or categorical values. 
Handling continuous treatment variables poses specific challenges, but there are standard approaches in causal inference to address them, such as propensity weighting~\cite{rosenbaum1983central} or variable discretization. 
We note that with continuous treatment variables, the search space for potential treatment patterns significantly expands, and thus, while the operation of the treatment mining algorithm remains consistent, the execution times increase.
Here, variable discretization may also be helpful, although this should be done cautiously to preserve the integrity of causal analysis. In our implementation, we did not discretize continuous variables, and we leave this optimization for future work.}




\textbf{Optional Changes:}
{\em All other comments/suggestions made by the reviewers.} \common{Please see the responses below.}



\cut{
\vspace{1mm}
This concludes the summary of the main revisions in the paper.
Below, you will find detailed responses to the reviewers' comments.
}



\vspace{1mm}
\noindent{\bf REVIEWER 1}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O1}} \emph{Consider a stronger justification for your assumptions, to make sure the proposed solution is practical (only AVG, no dependencies amongst tuples, single table).} \reva{
%{\bf Ans.}
% For supporting only the AVG aggregation function, we have revised the text in \cref{sec:franework} as detailed in Point 2.
\textbf{Ans.} Please see the changes detailed in {\bf Point 2} of the meta-review.
}
% We have revised the text in Section \ref{sec:franework} to justify our approach.  
% In particular, restricting to AVG is fundamental for causal explanations unlike non-causal methods.
% Our framework aims to find summarized \underline{\em causal explanations} for the query answers in $Q(D)$ using the concept of CATE discussed in Section~\ref{sec:prelim}. The causal estimates by CATE as shown in Eq.~(\ref{eq:cate}) and (\ref{eq:conf-cate}), inherently use {\em expectations, i.e., weighted average}. Thus, CATEs can be used when considering the aggregate average on the outcome column $Y$, e.g., ${\tt AVG(Salary)}$ in Example~\ref{ex:running_example}. Aggregate functions like {\tt SUM} or {\tt COUNT} depend on the {\em number of units} satisfying the conditions in Eq.~(\ref{eq:cate}) and (\ref{eq:conf-cate}), which does not have a correspondence with the estimate of causal effect (except that larger groups might reduce variance in the estimate). While other non-causal work on explanations or summarizations for query answers \cite{wu2013scorpion, roy2014formal, miao2019going, li2021putting, lakshmanan2002quotient, wen2018interactive} can support other aggregate functions, methods based on causal estimates focus on average as well \cite{salimi2018bias,youngmann2022explaining,abs-2207-12718}.


% As for the other assumptions, please see our response in Point 2 above. 


\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O2}} \emph{The tested baselines are not causal. Justify why there is no comparison with eg., [68] or [86]. Could you run them separately for each group and then somehow select the best explanations?} 
\reva{
%{\bf Ans.}
\textbf{Ans.} As mentioned in {\bf Point 1}, we added a causal baseline based on the framework in \cite{abs-2207-12718}.
We also revised {\bf \cref{sec:related}}, explaining why \cite{salimi2018bias, youngmann2022explaining} (old [68] and [86]) are not suitable baselines for our approach: 
Both these works propose using causal inference to explain query results. In particular, \cite{salimi2018bias} detects bias in a query in the form of confounder variables as explanations for the Simpson’s Paradox, while \cite{youngmann2022explaining} finds confounders that explain the correlation between the grouping attribute and AVG queries. In both, the treatment is the grouping attribute and is fixed, and the same explanation is provided for all groups. Here, we mine patterns as treatments and search for ones with strong causal effects for sets of groups. 
%, i.e., one of our goals is to find treatments.
}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O3}} \emph{clarify how IDS, FRL and ET were used in the experiments. One set of rules for the whole query? Separately for each group?}
\reva{
{\bf Ans.}
As we now clarify in {\bf \cref{subsec:setup}}, we gave \frl, \ids, and \exptable\ the input table, as they do not consider a SQL query, obtaining a single set of rules for the entire dataset. As mentioned in {\bf Point 1} in the meta-review, we also included another variant of \exptable\ that generates different explanations for sets of groups. The results are discussed in {\bf \cref{subsec:quality_eval}}.
}

\vspace{1mm}
\noindent{\bf REVIEWER 2}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.O1}} \emph{The treatment mining algorithm, rooted in the Apriori algorithm, shares similarities with many existing pattern mining algorithms. However, the uniqueness lies in the non-monotonic nature of the CATE value. The paper falls short in discussing the specific guarantees that this algorithm offers concerning its results, leaving room for questioning its reliability and effectiveness. Similarly, an in-depth discussion is absent for pattern mining, which may leave readers questioning the underlying principles.} 
\revb{
{\bf Ans.} 
As we now explain in the revised {\bf Section \ref{subsec:treatment_patterns}}, our treatment pattern mining algorithm leverages the notion of lattice traversal~\cite{DeutchG19,asudeh2019assessing}, to materialize and assess the CATE only for promising treatment patterns.
We do so by proposing a greedy approach that examines only nodes corresponding to treatments that are likely to have a positive CATE. In particular, we only materialize nodes if all their parents have a positive CATE. 
The primary distinction from existing solutions (e.g., ~\cite{asudeh2019assessing}) lies in the non-monotonic nature of CATE (meaning that adding a predicate to a treatment pattern can either increase or decrease its CATE). Consequently, exclusively materializing nodes where all of their parents exhibit a positive CATE might lead the algorithm to overlook certain relevant treatment patterns. However, according to our experiments (\cref{subsec:quality_eval}), combining treatment patterns that exhibit a positive CATE is highly likely to result in a treatment with a positive CATE as well. As a result, we managed to 
account for most treatments with a positive CATE, and the accuracy of this algorithm is relatively high.

As mentioned in {\bf Point 3} of the meta-review, we have revised the text in {\bf \cref{sec:algo}} to explain that both the grouping and the treatment mining algorithms can result in a non-optimal solution, as they prune patterns from consideration. 


Lastly, we have revised {\bf \cref{subsec:step_3}} to emphasize that the approximation guarantees of our LP formulation are solely theoretical since the approximation to the objective holds when \emph{all explanation patterns are considered}. In practice, we use the LP-rounding algorithm in conjunction with the grouping and treatment pattern mining procedures, therefore incurring a trade-off between value and efficiency and losing the theoretical guarantees.  
}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.O2}} \emph{The paper's decision to provide both positive and negative effects for the same pattern raises questions. The rationale behind this dual explanation for the same pattern is not made clear, leaving ambiguity about whether this is a mere byproduct of the algorithm or if it holds deeper significance in this specific application.} 
\revb{
{\bf Ans.}
Please refer to our response in {\bf Point 4} of the meta-review. 
}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.O3}} \emph{The experiments emphasize explanability and coverage, demonstrating that optimizations don't impair the explanations. However, there is a lack of clarity about how these measures translate into quality explanations. For example, the intuitive explanations presented in section 6.2 raise questions about the connection between quality and these specific measures. Additionally, it remains unclear whether the examples in this section were generated with optimization (brute-forced), leaving a gap in understanding the practical implications.} 
\revb{
{\bf Ans.}
In {\bf \cref{subsec:quality_eval}} we now emphasize that the explanations shown in {\bf \cref{fig:so-output-sensitive,fig:accidents}} were generated by the full \algoName\ algorithm. 
We have also revised {\bf Section \ref{subsec:problem}} to explain the rationale behind our problem formulation. 
Intuitively, our size and incomparability constraints ensure that the size of the explanation will be small with no redundancy and therefore it will be more easily grasped by users. The coverage constraint ensures that the explanation will be extensive and capture a significant part of the view, and the objective aims to maximize the validity of the explanation as the cause of the trends in the view. 
Further, as mentioned in {\bf Point 1} of the meta-review, we included experiments over synthetic data in which the ground truth (according to our definition) is known and evaluated whether \algoName\ can retrieve it (we report precision and recall of both grouping and treatments mining algorithms). 
}


\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.O4}} \emph{The description of the sampling algorithm is insufficient, leaving its impact on the quality of explanations ambiguous. This lack of detailed exposition could be a concern for readers attempting to comprehend the effect of sampling on explanations, thereby affecting their ability to fully grasp the framework's functionality and benefits} 
\revb{
{\bf Ans.}
Please see our response in {\bf Point 3} of the meta-review. Also, a full analysis of the effect of sampling on CATE value estimation and runtime is now given in the revised {\bf \cref{subsec:exp-sensitivity}}.
}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{Minor remarks}}\revb{
{\bf Ans.}
Thank you. We have fixed the typos (and proofread the paper to ensure there are no more typos).
}

\vspace{1mm}
\noindent{\bf REVIEWER 3}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.O1}} \emph{How CAUSUMX relates to and differs from the Query Result Explanation line of work needs further clarification. The authors mention that “those works are orthogonal to our work, as we aim to explain an entire aggregated view via a small set of causal explanations”. It’s unclear 1) what are the differences between explanations for the “entire view” versus explanations for query results, and 2) why can’t prior works be adapted to explain the entire view.} 
\revc{
{\bf Ans.}
We thank the reviewer for this comment. As we explain in the revised {\bf Section \ref{sec:related}}, \sysName\ generates a {\bf summarized} and \textbf{causal} explanation to the \textbf{entire aggregated view} generated by a SQL query while \textbf{accounting for variations among the groups.} In contrast, alternative approaches either provide non-causal explanations (as indicated in the Causal column of Table~\ref{tab:relatedwork}), focus solely on elucidating specific portions of query results (as evident in the Entire View column), or offer a single explanation for query results, neglecting differences among groups (as represented in the Support Groups column). 
Please also refer to our response for {\bf R1.O2}, for a discussion regarding the reasons why previous causal-based approaches cannot be adjusted to tackle the problem studied in our work.
}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.O2}} \emph{The evaluation does not include another causal baseline. In addition to showing the advantage of causal explanation over associations, it would also help to compare different forms of causal explanations to help justify the design choices and problem setup.} 
\revc{
{\bf Ans.}
We have added another causal-based baseline, namely \xinsight~\cite{abs-2207-12718}. Please refer to our response in {\bf Point 1} of the meta-review. 
}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.O3}} \emph{None of the baselines support group-bys... If grouping is the main limitation, can we run the explanation-table approach on grouping patterns generated by apriori?} 
\revc{
{\bf Ans.}
We thank the reviewer for this suggestion. We have added a comparison to a modified version of {\bf \exptable} \cite{Gebaly+2014-expltable} that includes a group-by query, and we compare against this version as well. Please see our response in {\bf Point 1} of the meta-review. 
}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.O4}} \emph{ It would help to include more quantitative measures on the quality and accuracy of the generated explanations. For example, the authors could use synthetic dataset with ground truth and report accuracy/recall, or perform user study with domain experts who can evaluate the quality of the generated explanations.} 
\revc{
{\bf Ans.}
Following the review's suggestion, we have included experiments over synthetic data and report precision and recall. Please see our response in {\bf Point 1} of the meta-review. 
}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.O5}} \emph{The underlying causal inference framework introduces some limitations to CAUSUMX, such as only supporting average functions. The assumption that tuples in the same table are independent is also non-trivial. The results also depend on the input casual DAG.} 
\revc{
{\bf Ans.}
Please refer to our response in {\bf Point 2} of the meta-review. 
}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.M1}} \emph{How does treatment mining deal with continuous variables? Do different discretization schemes affect the CATE values?} 
\revc{
{\bf Ans.}
Please refer to our response in {\bf Point 4} of the meta-review. 
}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.M2}} \emph{Is the redundant grouping pattern problem caused solely by functionally dependent columns? If so, the post-processing step is unnecessary as you can incorporate such constraints in apriori.} 
\revc{
{\bf Ans.}
Redundant grouping patterns can emerge even without functional dependencies among attributes. For example, the patterns \{HDI = High\} and \{GDP = High\} both identify the same set of tuples. Here, all countries with high HDI also have high GDP. However, two countries with medium HDI values may exhibit different GDP values. Thus, there is no functional dependency between HDI and GDP. Nevertheless, two grouping patterns defined by these attributes can lead to the same set of tuples, rendering the consideration of both redundant.
%We clarified this point in 
Please see the revised {\bf Section \ref{subsec:grouping_patterns}}.  
}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.M3}} \emph{What are runtime breakdowns among the three steps in CAUSUMX? I’m assuming that treatment pattern mining takes the longest.} 
\revc{
{\bf Ans.}
As we now mention in the revised {\bf Section~\ref{subsec:variants}}, a breakdown analysis by step of \algoName\ shows that in all cases, mining the treatment pattern phase consumes most of the time. The first and last steps are relatively fast. This aligns with our time complexity analysis. Full details are provided in the revised {\bf Section~\ref{subsec:variants}}.
}


==> sys.tex <==
\section{The \sysName\ System}




% \vspace{1mm}
% \noindent
% \textbf{Other Supported Functionalities}:
% The user can also restrict the attributes used to define the treatment patterns. This feature can be helpful for users seeking \emph{actionable recommendations}. For example, if a user departs from a particular city, they may not have control over certain factors, like the weather, but they can control other factors such as the airline carrier, time of the day/day of the week. In this case, the user may only be interested in explanations for high delays caused by the airline carrier and the time of the day and day of the week. Finally, users can also employ the system to assess the impact of treatment patterns of interest on the outcome. For instance, if a user departs from a particular city, she may want to evaluate the treatment effect of using a specific airline carrier or departing at a certain time of the day. 


